Open-world Instance Segmentation: Top-down Learning with Bottom-up Supervision

Many top-down architectures for instance segmentation achieve significant success when trained and tested on pre-defined closed-world taxonomy. However, when deployed in the open world, they exhibit notable bias towards seen classes and suffer from significant performance drop. In this work, we propose a novel approach for open world instance segmentation called bottom-Up and top-Down Open-world Segmentation (UDOS) that combines classical bottom-up segmentation algorithms within a top-down learning framework. UDOS first predicts parts of objects using a top-down network trained with weak supervision from bottom-up segmentations. The bottom-up segmentations are class-agnostic and do not overfit to specific taxonomies. The part-masks are then fed into affinity-based grouping and refinement modules to predict robust instance-level segmentations. UDOS enjoys both the speed and efficiency from the top-down architectures and the generalization ability to unseen categories from bottom-up supervision. We validate the strengths of UDOS on multiple cross-category as well as cross-dataset transfer tasks from 5 challenging datasets including MS-COCO, LVIS, ADE20k, UVO and OpenImages, achieving significant improvements over state-of-the-art across the board. Our code and models are available on our project page.

==> tables/rebuttalTable.tex <==
% \begin{table}[!t]
% \centering
%       \resizebox{0.25\textwidth}{!}{
%       \begin{tabular}{@{} l *{18}{c} @{}} 
%             \toprule 
%             % &  \multicolumn{2}{c}{Box AR} && \multicolumn{2}{c}{Mask AR} \\
%             & AR$_M^{100}$ & AR$_M^{300}$ \\
%             \cline{2-3}
%             MaskRCNN & 51.2 & 54.7 \\
%             UDOS & 46.4 & 50.7  \\
%             OLN & 47.4 & 50.8 \\
%             GGN & 49.2 & 52.7 \\
%             \bottomrule
%         \end{tabular}
%         }
%     \captionsetup{width=0.5\textwidth, font=footnotesize}
%     \caption{{Seen-class evaluation when trained and evaluated on all 80 COCO classes.} 
%     }
%     \label{tab:seen_classes}
%     \vspace{-16pt}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!t]
\centering
\resizebox{0.25\textwidth}{!}{
\begin{tabular}{@{} c *{18}{c} @{}}
\toprule
& MaskRCNN & UDOS & OLN & GGN \\
\cline{2-5}
AR$_M^{100}$ & 51.2 & 46.4 & 47.4 & 49.2 \\
AR$_M^{300}$ & 54.7 & 50.7 & 50.8 & 52.7 \\
\bottomrule
\end{tabular}
}
\captionsetup{width=0.45\textwidth, font=footnotesize}
\caption{{Seen-class evaluation on COCO dataset when trained and evaluated on all 80 COCO classes.}
}
\label{tab:seen_classes}
\vspace{-16pt}
\end{table}

==> tables/table.tex <==


\begin{table}[!t]
  \centering
  \resizebox{0.85\textwidth}{!}{
%   \rowcolors{6}{gray!25}{white}
% \centering
% \small
  \begin{tabular}{@{} l *{18}{c} @{}} 
    \toprule  \\[-1em]
    &  \multicolumn{6}{c}{Box AR} && \multicolumn{6}{c}{Mask AR} \\
    \cmidrule{2-7} \cmidrule{9-14}
    & AR10 & AR100 & AR300 & AR$_s$ & AR$_m$ & AR$_L$ && AR10 & AR100 & AR300 & AR$_s$ & AR$_m$ & AR$_L$ \\
    \midrule
    & \multicolumn{13}{c}{COCO $\rightarrow$ UVO} \\
    % Selective Search & - & - & - && - & - & - \\
    % Selective Search & - & 11.2 & 14.2 && - & 11.5 & 14.5 \\
    \cmidrule{2-14}
    % MaskRCNN & {11.3} & 25.2 & 31.1 && 9.3 & 20.6 & 25.5 \\
    % MaskRCNN$_b$ & - & 27.1 & - && - & 23.7 & - \\
    MaskRCNN$_s$ & 13.8 & 42 & 50.8 & 34.4 & 42.7 & 44.5 && 14.3 & 40.7 & 44.1 & 33.2 & 42.7 & 41.8 \\
    % \midrule
    OLN (ICRA'22) & 23.4 & 50.3 & 57.1 & 35.2 & 48.7 & 57.3 && \textbf{22 }& 41.4 & 44.7 & 29.5 & 42.3 & 45.1  \\
    % LDET (arxiv'21) & {21.5} & {34.8} & - && {19.7} & {31.0} & - \\
    % GGN (private) & - & 31.5 & - && - & 28.7 & - \\
    % \midrule
    Ours & \textbf{23.4} & \textbf{53.1} & \textbf{60.8} & 19.8 & 48.7 & 68.6 && 21.7 & \textbf{43.2} & \textbf{48.8} & 17.7 & 43.3 & 52.2  \\
    % Ours (with MCG) & 9.9 & 32.5 & {40.1} && 7.5 & {31.2} & {35.2} \\
    \bottomrule \\
  \end{tabular}
  }
    \caption{{\bf COCO to UVO transfer setting} Using 80 COCO categories to train and test on images from UVO containing images with open taxonomy.}
    \label{tab:voc2nvoc}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!t]
  \centering
  \resizebox{0.85\textwidth}{!}{
%   \rowcolors{6}{gray!25}{white}
% \centering
% \small
  \begin{tabular}{@{} l *{18}{c} @{}} 
    \toprule  \\[-1em]
    &  \multicolumn{5}{c}{Box AR} && \multicolumn{5}{c}{Mask AR} \\
    % \cmidrule{2-7} \cmidrule{9-14}
    & AR10 & AR100 & AR$_s$ & AR$_m$ & AR$_L$ && AR10 & AR100 & AR$_s$ & AR$_m$ & AR$_L$ \\
    \midrule
    & \multicolumn{11}{c}{COCO $\rightarrow$ ADE20k} \\
    % Selective Search & - & - & - && - & - & - \\
    % Selective Search & - & 11.2 & 14.2 && - & 11.5 & 14.5 \\
    \cmidrule{2-12}
    % MaskRCNN & {11.3} & 25.2 & 31.1 && 9.3 & 20.6 & 25.5 \\
    % MaskRCNN$_b$ & - & 27.1 & - && - & 23.7 & - \\
    MaskRCNN$_s$ & 5.3 & 19.1 & 15.4 & 21.2 & 21 && 5.3 & 18 & 14.3 & 20.2 & 19.6 \\
    % \midrule
    OLN (ICRA'22) & \textbf{9.3} & 24.7 & 15.7 & 27.8 & 31.6 && \textbf{8.5 }& 20.4 & 13.3 & 23.2 & 25.2 \\
    % LDET (arxiv'21) & {21.5} & {34.8} & - && {19.7} & {31.0} & - \\
    % GGN (private) & - & 31.5 & - && - & 28.7 & - \\
    % \midrule
    Ours & 8.9 & \textbf{26.8} & 11 & 26.6 & 45.4 && 8.0 & \textbf{22.6} & 9.7 & 23.2 & 36.5  \\
    % Ours (with MCG) & 9.9 & 32.5 & {40.1} && 7.5 & {31.2} & {35.2} \\
    \bottomrule \\
  \end{tabular}
  }
    \caption{{\bf COCO to ADE20k transfer setting} Using 80 COCO categories to train and test on images from ADE20k containing annotations for both stuff and thing classes.}
    \label{tab:voc2nvoc}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!t]
  \centering
  \resizebox{0.85\textwidth}{!}{
%   \rowcolors{6}{gray!25}{white}
% \centering
% \small
  \begin{tabular}{@{} l *{18}{c} @{}} 
    \toprule  \\[-1em]
    &  \multicolumn{6}{c}{Box AR} && \multicolumn{6}{c}{Mask AR} \\
    \cmidrule{2-7} \cmidrule{9-14}
    & AR10 & AR100 & AR300 & AR$_s$ & AR$_m$ & AR$_L$ && AR10 & AR100 & AR300 & AR$_s$ & AR$_m$ & AR$_L$ \\
    \midrule
    & \multicolumn{13}{c}{COCO $\rightarrow$ OpenImages} \\
    % Selective Search & - & - & - && - & - & - \\
    % Selective Search & - & 11.2 & 14.2 && - & 11.5 & 14.5 \\
    \cmidrule{2-14}
    MaskRCNN & 20.5 & 41.1 & 49.7 & 17.3 & 29.8 & 44.2 && 20.3 & 40.4 & 44.2 & 13.8 & 30.7 & 43.2 \\
    % MaskRCNN$_b$ & - & 27.1 & - && - & 23.7 & - \\
    MaskRCNN$_s$ & 25 & 54.1 & 59.1 & 20.6 & 41 & 57.8 && 25.1 & 54.2 & 57.4 & 17.7 & 41.0 & 58.0 \\
    % \midrule
    OLN (ICRA'22) & 41.7 & 64.1 & 68.4 & 22.8 & 47.5 & 68.8 && 39.9 & 60.0 & 63.5 & 15.2 & 41.8 & 65.1  \\
    % LDET (arxiv'21) & {21.5} & {34.8} & - && {19.7} & {31.0} & - \\
    % GGN (private) & - & 31.5 & - && - & 28.7 & - \\
    % \midrule
    Ours & \textbf{48.8} & \textbf{71.6} & 74.6 & 13.9 & 47.3 & 78.4 && \textbf{47.0} & \textbf{66.2} & 68.7 & 9.2 & 44.4 & 72.0  \\
    % Ours (with MCG) & 9.9 & 32.5 & {40.1} && 7.5 & {31.2} & {35.2} \\
    \bottomrule \\
  \end{tabular}
  }
    \caption{{\bf COCO to OpenImages transfer setting} Using 80 COCO categories to train and test on images from OpenImages containing many categories from outside COCO taxonomy.}
    \label{tab:voc2nvoc}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!t]
  \centering
  \resizebox{0.85\textwidth}{!}{
%   \rowcolors{6}{gray!25}{white}
% \centering
% \small
  \begin{tabular}{@{} l *{18}{c} @{}} 
    \toprule  \\[-1em]
    &  \multicolumn{6}{c}{Box AR} && \multicolumn{6}{c}{Mask AR} \\
    \cmidrule{2-7} \cmidrule{9-14}
    & AR10 & AR100 & AR300 & AR$_s$ & AR$_m$ & AR$_L$ && AR10 & AR100 & AR300 & AR$_s$ & AR$_m$ & AR$_L$ \\
    \midrule
    & \multicolumn{13}{c}{COCO $\rightarrow$ LVIS} \\
    % Selective Search & - & - & - && - & - & - \\
    % Selective Search & - & 11.2 & 14.2 && - & 11.5 & 14.5 \\
    \cmidrule{2-14}
    MaskRCNN & 4.9	& 19.4 & 26	& 12.6 & 31.5 &	40.4	&&	4.1 & 16.6	& 22.2	& 10.7 & 28.6 & 29.4 \\
    % MaskRCNN$_b$ & - & 27.1 & - && - & 23.7 & - \\
    MaskRCNN$_s$ & 5.6	& 21.9 & 28.1 & 17.1 & 31.7 & 32.9 && 5.6 & 20.8 & 24.3 & 15.7 & 32.2 & 28.7 \\
    % \midrule
    OLN (ICRA'22) & \textbf{8.9}	& \textbf{26}	& \textbf{32.1}	&18	&40.8	&48.5&&		\textbf{8.5}	&\textbf{22.8}	&\textbf{27}	&16.2&	36.7	&35.4  \\
    % LDET (arxiv'21) & {21.5} & {34.8} & - && {19.7} & {31.0} & - \\
    % GGN (private) & - & 31.5 & - && - & 28.7 & - \\
    % \midrule
    Ours & 5.5 & 20.7 & 30.8 & 8 & 42.4 & 62.7 && 5	& 18.1 & 26.6 & 6.8 & 39.4 & 48.6  \\
    % Ours (with MCG) & 9.9 & 32.5 & {40.1} && 7.5 & {31.2} & {35.2} \\
    \bottomrule \\
  \end{tabular}
  }
    \caption{{\bf COCO to LVIS transfer setting} }
    \label{tab:voc2nvoc}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[!t]
  \centering
  \resizebox{0.6\textwidth}{!}{
%   \rowcolors{6}{gray!25}{white}
% \centering
% \small
  \begin{tabular}{@{} l *{5}{c} @{}} 
    \toprule  \\[-1em]
    &  \multicolumn{4}{c}{Box AR} \\
    & AR100 & AR$_S$ & AR$_M$ & AR$_L$  \\
    \midrule
    Ours (w/o grouping) & 48.4 & 25.1 & 50.3 & 55.7 \\
    Ours (with grouping) & 53.1 & 22.3 & 49.6 & 67.3 \\
    \bottomrule \\
  \end{tabular}
  }
    \caption{{\bf Effect of grouping} Grouping vs. no grouping on UVO val set.}
    \label{tab:voc2nvoc}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[!t]
  \centering
  \resizebox{0.6\textwidth}{!}{
%   \rowcolors{6}{gray!25}{white}
% \centering
% \small
  \begin{tabular}{@{} l *{6}{c} @{}} 
    \toprule  \\[-1em]
    &  \multicolumn{2}{c}{Box AR} && \multicolumn{2}{c}{Mask AR} \\
    & AR100 & AR300 && AR100 & AR300  \\
    \cline{2-3} \cline{5-6}
    % \midrule
    Selective Search & {31.9} & {40.0} && {29.4} & {32.9} \\
    MCG & 31.1 & {40.3} && {30.0} & {35.9} \\
    SSN & 18.1 & 24.3 && 18.0 & 21.2 \\
    Grid & 15.0 & 21.6 && 15.1 & 19.6 \\
    \bottomrule \\
  \end{tabular}
  }
    \caption{{\bf Effect of super-pixels} Different types of super-pixels used.}
    \label{tab:voc2nvoc}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
